Randomized Wagering Mechanisms

Wagering mechanisms are one-shot betting mechanisms that elicit agents' predictions of an event. For deterministic wagering mechanisms, an existing impossibility result has shown incompatibility of some desirable theoretical properties. In particular, Pareto optimality (no profitable side bet before allocation) can not be achieved together with weak incentive compatibility, weak budget balance and individual rationality. In this paper, we expand the design space of wagering mechanisms to allow randomization and ask whether there are randomized wagering mechanisms that can achieve all previously considered desirable properties, including Pareto optimality. We answer this question positively with two classes of randomized wagering mechanisms: i) one simple randomized lottery-type implementation of existing deterministic wagering mechanisms, and ii) another family of simple and randomized wagering mechanisms which we call surrogate wagering mechanisms, which are robust to noisy ground truth. This family of mechanisms builds on the idea of learning with noisy labels (Natarajan et al. 2013) as well as a recent extension of this idea to the information elicitation without verification setting (Liu and Chen 2018). We show that a broad family of randomized wagering mechanisms satisfy all desirable theoretical properties.

==> app.tex <==
%%appendix
\newpage
%\section*{High probability guarantee with less conservative scaling}
%We first note that when the number of agent is large, the second score term $\sum_{j \in N\backslash \{i\}} \frac{w_j}{W_{N}} \varphi \circ s_{\tilde{x}_j}(p_j)$ converges to its expectation that
%\[
%\sum_{j \in N\backslash \{i\}} \frac{w_j}{W_{N}} \varphi \circ s_{\tilde{x}_j}(p_j) \rightarrow \sum_{j \in N\backslash \{i\}} \frac{w_j}{W_{N}} s_{x}(p_j)
%\]
% Then the worst case score of $\varphi \circ \Pi^{\text{WS}}_i(\cdot)$ becomes roughly
% \[
%\varphi \circ \Pi^{\text{WS}}_i(\cdot) \geq  w_i \bigl(\frac{-e_{1-\tilde{x}_i}}{1-e_0-e_1} -1 \bigr). %= \frac{e_1-1}{1-e_0-e_1}w_1
%\]
%Then we can set $b$ to be
%\[
%b = \max\bigl\{ \frac{1-e_0}{1-e_0-e_1},  \frac{1-e_1}{1-e_0-e_1}\bigr\}
%\]
%This is a better rescaling compared to the one we give in the previous section - but the budget feasibility holds only with high probability. We will show in simulation that this change is already enabling us to achieve much better money exchange property compared to the deterministic wagering mechanisms. Though again, we still suffer from the first drawback that the expected payment drops proportionally in $b$.
%
%We can use Hoeffding inequality to easily bound it:
%\begin{theorem}\label{HPB:CON}
%With probability at least $1-\frac{1}{N^2}$, 
%\[
%\sum_{j \in N\backslash \{i\}} \frac{w_j}{W_{N}} \varphi \circ s_{\tilde{x}_j}(p_j)  -  \sum_{j \in N\backslash \{i\}} \frac{w_j}{W_{N}} s_{x}(p_j) < 2b \sqrt{\sum_{j \neq i} (\frac{w_j}{w_N})^2} \cdot \sqrt{\log N}. 
%\]
%\end{theorem}
%Note: when there is no monopoly agents such that $\frac{w_j}{w_N} = \Theta(\frac{1}{N})$, we will have 
%\[
%\sqrt{\sum_{j \neq i} (\frac{w_j}{w_N})^2} \cdot \sqrt{\log N} = \Theta(\sqrt{\frac{\log N}{N}}) \rightarrow 0.
%\]
%
%\begin{proof}
%Using Hoeffding inequality we know that
%\begin{align*}
%&\Pr \biggl[ \sum_{j \in N\backslash \{i\}} \frac{w_j}{W_{N}} \varphi \circ s_{\tilde{x}_j}(p_j) - \mathbb E\bigl[ \sum_{j \in N\backslash \{i\}} \frac{w_j}{W_{N}} \varphi \circ s_{\tilde{x}_j}(p_j)\bigr] \geq \delta \bigr] \\
%\leq &\text{exp}\biggl( -\frac{2\delta^2}{\sum_{j \neq i} (b\cdot \frac{w_j}{W_N} - (-b\frac{w_j}{W_N}))}\biggr)\\
%=& \text{exp}\biggl( -\frac{2\delta^2}{4b^2 \sum_{j \neq i} \frac{w^2_j}{W^2_N}}\biggr). %\leq \text{exp}\bigl( -\frac{2\delta^2}{4b^2}\bigr).
%\end{align*}
%The last inequality is due to the fact that
%\[
%W^2_N \geq \sum_{j \neq i} w^2_j.
%\]
%Then the theorem is proved by setting $\delta:=2b\sqrt{\sum_{j \neq i} (\frac{w_j}{w_N})^2} \cdot \sqrt{\log N}$, and using the fact that %$\delta:=2b\sqrt{\log N}$.
%\[
% \mathbb E\biggl[ \sum_{j \in N\backslash \{i\}} \frac{w_j}{W_{N}} \varphi \circ s_{\tilde{x}_j}(p_j)\biggr] = \sum_{j \in N\backslash \{i\}} \frac{w_j}{W_{N}} s_{x}(p_j).
%\]
%\end{proof}


\section*{{\LARGE SUPPLEMENTAL MATERIAL}}
~\\

\section{Other related work} 

%\begin{itemize}
%\item proper scoring rule, wagering mechanism. learning with noisy data
%\end{itemize}

%Needed references:
%\begin{itemize}
%\item \textsf{WSWM} and its journal version: \cite{lambert2008self,lambert2015axiomatic}
%\item \textsf{NAWM}: \cite{chen2014removing}. Double Clinching Auction Wagering: \cite{freeman2017double}. Parimutuel \cite{Johnstone:2007,Plott97,Tha:88,Agrawal:08}. Proxy parimutuel \cite{Win:68b}.
%\item Strictly proper scoring rules: \cite{gneiting2007strictly}. Brier scoring rule: \cite{Brier:50}. Competitive scoring rule: \cite{Kilgour:04}.  Experimental studies: \cite{Nelson:89}.
%\item Scoring rule \cite{Jose:06,Matheson:76,Win:69}
%\item information market \cite{Chen:05a,Chen:06a}
%\item learning with noisy data: \cite{natarajan2013learning,scott2015rate}
%\end{itemize}

The ability to elicit \emph{information}, in particular predictions and forecasts about future events, is crucial for many application settings and has been studied extensively in the literature. Proper scoring rules have been designed \citep{Brier:50,Jose:06,Matheson:76,Win:69,gneiting2007strictly} for this purpose, where each agent is rewarded by how well their reported forecasts predicted the true realized outcome (after the outcome is resolved). Later, competitive scoring rule \citep{Kilgour:04} and a parimutuel Kelly probability scoring rule \citep{Johnstone:2007} adapt proper scoring rules to group competitive betting. Both mechanisms are budget balanced so that the principal doesn't need to pay any participant. These spur the further development of the previously discussed wagering mechanisms \citep{lambert2008self,lambert2015axiomatic,chen2014removing,freeman2017double,freeman2018axiomatic} and the examination of their theoretical properties.  

%In order to implement a scoring system for prediction collection, the mechanism designer needs to pre-allocate a set of budgets to cover an certain amount of rewards to offer. Later, a competitive scoring rule was introduced in \cite{Kilgour:04} to adapt the existing scoring rules to a fixed budget one. The idea is that each agent will be rewarded according to how better each agent is predicted compared to others. The solution can be read as a allocation of the total fixed budget based on each agent's relative performance. 

%The above idea is further developed into a family of self-financed mechanisms, jointly called wagering mechanism, where agents first wager in a certain amount of money that they are willing to loss, and then the mechanism designer will decide a reallocation of the total wager according to their forecast accuracy and wagers.  \cite{lambert2008self,lambert2015axiomatic} proposed a weighted scoring rule based wagering mechanism and showed that this class of mechanisms is unique up to satisfying a set of desirable properties. The above mechanism is later extended to a non-arbitrage version where opportunity of agents risklessly making profits is removed \cite{chen2014removing}. However, both of above two wagering mechanisms suffer from Pareto inefficiency, that is there exist profitable side bets for each agent. Nothing this issue, a double clinching auction based wagering mechanism is proposed in \cite{freeman2017double} and is shown to able to significantly improve the Pareto efficiency. However, it is established in \cite{freeman2017double} an impossibility result that there does not exist a deterministic wagering mechanism that is Pareto optimal and satisfies a set of desirable properties at the same time.

Our method used in lottery wagering mechanisms to transfer an arbitrary deterministic wagering mechanism into a randomized one, while maintaining the properties, is inspired by the method proposed in \citep{witkowski2018incentive}. The paper studies the incentive compatible forecasting competition and it transfers scores of multiple predictions into the odds of winning to maintain properties of the scoring rules. \citep{lambert2008self}  proposed a randomization method based on \textsf{WSWM} via randomly selecting strictly proper scoring rules and proper scoring rules with extreme values to increase the stake.  However, this method does not generalize to other deterministic wagering mechanisms.  \citep{cummings2016possibilities} proposed to apply differential privacy technology to randomize the payoff of wagering mechanisms in order to preserve the privacy of each agent's belief. However, their method does not maintain budget balance (in ex-post).

Our method of defining an unbiased operator to remove the bias introduced by randomness in \textsf{SWM} is inspired by techniques used in Machine Learning, in particular the literature on learning with noisy labels \citep{bylander1994learning,natarajan2013learning,scott2015rate}. This idea has been recently used to design surrogate scoring rules \citep{SSR}. We demonstrate yet another application of this powerful tool in wagering mechanism design.

%\red{To do: a summary of properties of mechanisms including WSWM, NAWM, DCA, PCM, LWM, SWS (and Randomized WSWM in Lambert 2008?) somewhere in the paper.}
We summarize the properties of existing wagering mechanisms in Table~\ref{property_table}.
\begin{table}[h!]
  \begin{center}
    \caption{A summary of properties of wagering mechanisms\label{property_table}}
    \label{tab:table1}
    \begin{tabular}%{|c|c|p{1.6cm}|p{1.9cm}|p{1.5cm}|p{1.5cm}|p{1.4cm}|p{1.5cm}|} 
{|c|c|c|c|c|} 
    \hline
      & \textbf{Budget} & \textbf{Incentive} & \textbf{Pareto} &  \textbf{No}  \\
      Mechanism &  \textbf{Balance} & \textbf{Compatibility} & \textbf{Optimality}  & \textbf{Arbitrage}
      \\
      \hline
      \textsf{WSWM}~\cite{lambert2008self} & Strictly&  Strictly & \textbf{False}
     & \textbf{False} \\\hline
      \textsf{NAWM}~\cite{chen2014removing} & \textbf{Weakly} &  Strictly & \textbf{False}  & True \\\hline
      \textsf{DCA}~\cite{freeman2017double} & Strictly &  \textbf{Weakly} & \textbf{False}  & True \\\hline
      \textsf{PCM}~\cite{freeman2018axiomatic} & Strictly &  \textbf{False} & True & True \\\hline
      Randomized \textsf{WSWM}~\cite{lambert2008self} & Strictly &  True & \textbf{False} &   True\\\hline
      Private \textsf{WSWM}~\cite{cummings2016possibilities}& \textbf{False} &  True &  \textbf{False} &  True\\\hline
      \textsf{LWS} (this paper) & Strictly &  True & True & True\\\hline
      \textsf{RP-SWME} (this paper) & Strictly &  True & True & True
      \\\hline
      %\textsf{LWS} & Strictly & True & Strictly & True & True & True & True\\\hline
      %\textsf{RP-SWME} & Strictly & True & Strictly & True & True & True & True\\\hline
    \end{tabular}
  \begin{tabular}{l}
  (All of the mechanisms in this table satisfy individual rationality, anonymity, neutrality and sybilproofness.)
  \end{tabular}
  \end{center}

\end{table}

\section{Missing definition and proof}
\subsection{Definition of Anonymity and Neutrality}

Anonymity requires that agents' identities do not affect their net-payoffs. Let $\sigma_\mathcal{N}$ be a permutation of the set of agents $\mathcal{N}$, and denote $\hp_{\sigma_\mathcal{N}}, \bw_{\sigma_\mathcal{N}}$ the reports and wagers of agents after applying the permutation respectively. Denote $\mathcal{D}_{\sigma_\mathcal{N}}$ the joint distribution of net-payoffs of agents in $\mathcal{N}$ after applying the permutation on agents.
\begin{definition}
A randomized wagering mechanism is \textbf{anonymous} if 
$\forall \sigma_\mathcal{N}, \hp,\bw,x: \mathcal{D}(\hp;\bw;x)=\mathcal{D}_{\sigma_\mathcal{N}}(\hp_{\sigma_\mathcal{N}};\bw_{\sigma_\mathcal{N}};x)$
\end{definition}


%\textbf{Anonymity}: Agents' identities do not affect their net-payoffs: that is for all $\report{},\mathbf{w}$ and all permutation $\sigma$ defined on the set of $N$ participating agents, we have: 
%$f^{\mathcal D(\report{\sigma},\mathbf{w}_{\sigma}, x)}(\pi_{\sigma}) = f^{\mathcal D(\report{},\mathbf{w}, x)}(\pi).$

Neutrality requires that the net-payoffs do not depend on the labeling of the event outcomes.
Let $\sigma_\mathcal{M}$ be a permutation of the set of outcomes $\mathcal{M}$. Denote by $\hp_i^{\sigma_\mathcal{M}}$ the reported prediction of agent $i$ after we relabel the outcomes according to permutation $\sigma_\mathcal{M}$, and denote by $\sigma_\mathcal{M}(x)$ the new label of an outcome $x\in\mathcal{M}$.

\begin{definition}
A randomized wagering mechanism is \textbf{neutral} if $\forall \sigma_\mathcal{M}, \hp,\bw,x:$
$$
\mathcal{D}(\hp;\bw;x)=\mathcal{D}(\hp_1^{\sigma_\mathcal{M}},...,\hp_N^{\sigma_\mathcal{M}};\bw;\sigma_\mathcal{M}(x)).
$$
\end{definition}

%\section*{Proof of Theorem \ref{THM:PO}}
%\begin{proof}
%\underline{Sufficiency (``if", $\Leftarrow$)}: Obviously, if no inequality holds, there exists no extra wagers for a side bet. If there exists a set agents with  $\pi_i <w_i$ and $p_i = p$ for some  $p\in[0,1]$, for any (weakly) budget balance mechanism, the budget balance condition implies that the sum of the expected utilities of all these agents, according their common report $p$, is no more than 0, showing that no one can benefit without harming another. Thus, a profitable set bet does not exist.\\
%\underline{Necessity (``only if", $\Rightarrow$)}:  We prove by contradiction. Suppose there exist two agents $i$ and $j$, such that $\pi_i<w_i$, $\pi_j<w_j$ and $p_i\ne p_j$, then it can be easily checked that \textsf{WSWM} with input profile $(p_i, p_j, w_i, w_j)$ is a profitable side bet.
%\end{proof}

\subsection{Proof of Theorem~\ref{thm_lwm}}
\begin{proof}
 \textsf{LWS} satisfies (a) - (f) immediately as the expected payoff of \textsf{LWS} of each agent equals to his payoff under \textsf{WSWM} and the payoff in total in any case also equals to the payoff in total under \textsf{WSWM}. 

Next, we prove that \textsf{LWS} satisfies (g). In \textsf{WSWM}, if the number of agents is finite, no agent can lose all his money regardless of the event outcome~\cite{lambert2008self}. As a result, no agent can win all the wagers no matter which of the event outcomes is realized. Therefore, in \textsf{LWS}, no agent can be the winner with probability 1 regardless of the event outcome, meaning that any agent always has a positive probability to lose all his wager and no agent can risklessly make profits.

\textsf{LWS} satisfies (h) because in all cases, only one agent has a positive payoff, and all the other agents lose all their wagers, leaving them no budget for a profitable side bet.

\end{proof}

%\section*{Affine transformation of \textsf{SWM}}


\subsection{Proof of Lemma~\ref{sws:er}}
\begin{proof}
In this proof, we use Brier Score as the scoring rule used by the mechanism, i.e., $s_x(\hat{p}_i)=1-(x-\hat{p}_i)^2$, and $\hat{p}_i$ is agent $i$'s report of $\mathbb{P}(X=1)$. The proof can be extended to other strictly proper scoring rule within [0, 1].

We first consider the corner case where all agents reports 0.5. It can be verified that in Algorithm 2, $\min_{i\in\mathcal{N}} r_i=0.5$, and the algorithm sets $e_0^i=e_1^i=0,\forall i$ and \textsf{SWME} is reduced to \textsf{WSWM}. Thus, no wager violation happens.

Next, we consider the scenario that $\exists i\in\mathcal{N}, \hat{p}\ne 0.5$. In this scenario, we first prove that, in Algorithm 2 $\forall i, r_i\in(0,0.5)$.

We have  $\forall i, s_i^w, s_i^b\in[0,1], s_i^w\le s_i^b$ (the equality only holds when $\hat{p}_i=0.5$), $s_i^w+s_i^b\in [0.5, 1]$. 
Let 
$$A=(1-\frac{w_i}{W_\mathcal{N}})s_i^w-\sum_{j\in\mathcal{N}\backslash\{i\}}\frac{w_j}{W_\mathcal{N}}s_j^b$$ 
and 
$$B=(1-\frac{w_i}{W_\mathcal{N}})(s_i^w+s_i^b)-\sum_{j\in{\mathcal{N}\backslash\{i\}}}\frac{w_j}{W_\mathcal{N}}(s_j^w+s_j^b).$$
We have $r_i=\frac{1}{2}+\frac{2A-B}{2(2+B)}$, $A>-1, B\in (-1,1)$ and $2A-B = \sum_{j\in \mathcal{N}\backslash\{i\}}\frac{w_j}{W_\mathcal{N}}(s_j^w-s_j^b)+(1-\frac{w_i}{W_{\mathcal{N}}})(s_i^w-s_j^b)> 0$ (there exists at least one agent $i\in\mathcal{N}$ that $\hat{p}_i\ne 0.5$). Therefore, $\frac{2A-B}{2+B}\in(-1, 0)$. We have $r_i=\frac{1}{2}+\frac{2A-B}{2(2+B)}\in(0, 0.5)$.

Next, we prove that if let $r_i$ be a variable, and let $e_0^i=e_1^i=r_i$, the worst cast net-payoff $\pi^w_i$ (w.r.t. the event outcome and the randomness of the mechanism) of agent $i$ is a decreasing function of $r_i$.

In the worst case of agent $i$, $\varphi \circ s_{\tilde{x}_i}(\hat{p}_i) = \frac{(1-r_i)s_i^w-r_is_i^b}{1-2r_i}, \varphi \circ s_{\tilde{x}_j}(\hat{p}_j) = \frac{(1-r_i)s_i^b-r_is_i^w}{1-2r_i}$ and $\pi^w_i = w_i\frac{(A-Br_i)}{1-2r_i}$. We have $\frac{\partial \pi_i^w}{\partial r_i} = w_i\frac{2A-B}{(1-2r_i)^2}<0$. Therefore, $\pi_i^w$ is decreasing with $r_i$.

Finally, it is easy to verify that when $r_i=\frac{1}{2}+\frac{2A-B}{2(2+B)}$, $\pi_i^w=-w_i$.

Therefore, when we set for each agent $i\in\mathcal{N}$, $e_i^0=e_i^1=\min_{j\in\mathcal{N} }r_j$, no agent can lose more than his wager and agent $i^*=\text{argmin}_{j\in{\mathcal{N}}} r_j$ loses all his wager in the worst case. 
\end{proof}

\input{property}


%\section*{Proof of Lemma~\ref{LM:SYB}}
%\begin{proof}
%We prove the claim for the case that an agent is only allowed to create two identities. The claim holds in general, as we can alway merge two identities into one without decreasing the payoff, following the result of the case of two. 
%
%Fixing an arbitrary belief $\mathbf{p}_i$ of agent $i$, we denote the $E_i^{\mathcal W}(\report{},\mathbf{w}):=\mathbb{E}_{X\sim\mathbf{p}_i, \mathcal{D}^{\mathcal W}(\report{},\mathbf{w},X)}[\Pi_i(\report{},\mathbf{w},X=x)] $, where $\mathcal{D}^{\mathcal W}(\cdot)$ is the distribution specified by mechanism $\mathcal W$. 
%Suppose an agent $i$ divides its wager $w_i$ into two wagers   $w_{i1}, w_{i2}$, and reports two predictions $\report{i1}, \report{i2}$ correspondingly. 
%We have $\forall \report{i1}, \report{i2}, w_{i1}, w_{i2}, \report{-i}, \mathbf{w}_{-i}, x$, 
%\begin{small}
%\begin{align*}
%& E_i^{\mathcal W*}(\report{i1}, \report{i2},  \report{-i}, w_{i1}, w_{i2}, \mathbf{w}_{-i})  \\
%=  &  \sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\report{i1}, \report{j}, w_{i1}, w_j) +\sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\report{i2}, \report{j}, w_{i2}, w_j) 
%+
% \frac{1}{N}\left(E_{i1}^{\mathcal W}(\report{i1}, \report{i2}, w_{i1}, w_{i2}) + E_{i2}^{\mathcal W}(\report{i1},\report{i2},w_{i1}, w_{i2})\right) \\
%\le & \sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\report{i1}, \report{j}, w_{i1}, w_j) +\sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\report{i2}, \report{j}, w_{i2}, w_j) 
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,  
%(\mathcal W\text{ is (weakly) budget balance})\\
%\le & \sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\mathbf{p}_i, \report{j}, w_{i1}, w_j) +\sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\mathbf{p}_i, \report{j}, w_{i2}, w_j) 
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,
% (\mathcal W\text{ is (weakly) incentive compatible})\\
%\le & \sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\mathbf{p}_i, \report{j}, w_{i}, w_j) 
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, \,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, 
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,
% (\mathcal W\text{ is sybilproof})\\
%\le &  \sum_{j\ne i} \frac{1}{N-1}E_i^{\mathcal W}(\mathbf{p}_i, \report{j}, w_{i}, w_j) =  E_i^{\mathcal W*}(\mathbf{p}_i, \report{-i}, w_{i}, \mathbf{w}_{-i})
%\end{align*}
%\end{small}
%Therefore,  $\mathcal W*$ is sybilproof.
%\end{proof}





%\section*{Other properties of \textsf{SWS}}
%\emph{Incorporating agent risk preference} Note that each $\Pi^{\text{SWS}}_i(\cdot)$ is linear in $s_{\tilde{x}_j}(p_j)$. So the idea of surrogate loss function can be applied to each agent's flipped outcome separately with different error rates. Therefore our mechanism is able to incorporate different agents' preferences. When agents prefers risk, we can tune its error rate higher; on the other hand, when agent prefers no risk, we can set his error rate low. 


\section{Extensions of \textsf{SWM}}

We discuss a couple of useful extensions of \textsf{SWM}: i). one is instead of building on $\textsf{WSWM}$, we show the idea of surrogate idea can also build upon another deterministic wagering mechanism $\textsf{NAWM}$. (ii). We extend our results to a multi-outcome setting. 

\subsection{Surrogate \textsf{NAWM}}\label{sec:snawm}

We note that the bias removal procedure adopted in \textsf{SWM} does not rely the specific underlying wagering mechanism heavily. We demonstrate the idea with a non-arbitrage wagering mechanism (\textsf{NAWM}, \citep{chen2014removing})\footnote{Though the randomization device already grants us the non-arbitrage property, we pick this mechanism for i. its simplicity for presentation, as \textsf{NAWM} also extends from \textsf{WSWM}. ii. we will show in experiments later that we empirically observe higher risk when applying this surrogate based randomized \textsf{NAWM}. }. 

%\begin{itemize}
%\item Randomly flip the outcome for each agent to obtain $\outcome{}$ as we detailed ealier.  
%\item Compute each agent $i$'s payoff function as follows:
%\begin{align}
%\varphi \circ \Pi^{\text{NA}}_i(p_i,\mathbf{p}_{-i},\mathbf{w},\tilde{x}) =\frac{w_i W_{N\backslash \{i\}}}{W_{N}}\biggl( \varphi \circ s_{\tilde{x}_i}(p_i) -  \varphi \circ s_{\tilde{x}_i}(\bar{p}(\report{-i},\mathbf{w}_{-i}))\biggr),
%\end{align}
%where $\bar{p}$ is a real-value function defined in \citep{chen2014removing}.
%\end{itemize}
%
%The extension should be clear from above formulation as $\varphi \circ \Pi^{\text{NA}}_i(\cdot)$ is in effect a linear combination of $s_{\tilde{x}_i}(p_i) $ and $s_{\tilde{x}_i}(\bar{p}(\report{-i},\mathbf{w}_{-i}))$ so the unbiaseness property will hold. 

Notice that since $\Pi^{\text{NA}}_i(\cdot)$ is not linear in the surrogate scores of each agent, the budget balance argument is not as easy as in the \textsf{WSWM} case. Nonetheless we notice the following fact proved in \citep{chen2014removing}:
\[
\Pi^{\text{NA}}_i(\hat{p}_i,\mathbf{\hat{p}}_{-i},\mathbf{w},X=x) = \Pi^{\text{WS}}_i(\hat{p}_i,\mathbf{\hat{p}}_{-i},\mathbf{w},X=x) -  \Pi^{\text{WS}}_i(\bar{\hat{p}}_i,\mathbf{\hat{p}}_{-i},\mathbf{w},X=x)
\]
where $\bar{\hat{p}}_i$ denotes the average prediction from $j \neq i$. Then we can safely apply the surrogate idea to the first \textsf{WSWM} scoring term:
\[
\varphi \circ \Pi^{\text{NA}}_i(\hat{p}_i,\mathbf{\hat{p}}_{-i},\mathbf{w},\tilde{\mathbf{X}}=\outcome{}) = \varphi \circ \Pi^{\text{WS}}_i(\hat{p}_i,\mathbf{\hat{p}}_{-i},\mathbf{w},\tilde{\mathbf{X}}=\outcome{})-  \Pi^{\text{WS}}_i(\bar{\hat{p}}_i,\mathbf{\hat{p}}_{-i},\mathbf{w},X=x)
\]
This mechanism will enjoy the higher risk property introduced by surrogate wagering, as well as the non-arbitrage (in conditional expectation) brought in by \textsf{NAWM}. 


\subsection{Multi-outcome events}
\label{non-binary}

For simplicity, our previous discussions focused largely on the binary outcome scenario. As promised, we now show that our results extend to the non-binary events. Recall that there are $M$ outcomes, denoting as $[0,1,2,...,M-1]$. Denote the following confusion matrix
\[ C = 
\begin{bmatrix}
    c_{0,0}       & c_{0,1} &  \dots & c_{0,M-1} \\
    c_{1,0}        & c_{1,1}  & \dots & c_{1, M-1} \\
    \hdotsfor{4} \\
    c_{M-1,0}       & c_{M-1,1} & \dots & c_{M-1,M-1}
\end{bmatrix}
\]
and each entries $c_{j,k}$ indicates the flipping probability for generating a surrogate outcome:
$
c_{j,k} = \Pr[\tilde{X}_i = k|X=j].
$

The core challenge of this extension is to find an unbiased operator $\varphi$. Writing out the conditions for unbiasedness (s.t. $\mathbb E_{\tilde{X}_i|x}[\varphi \circ s_{\tilde{X}_i=\tilde{x}_i}(\mathbf{\hat{p}})] = s_{x}(\mathbf{\hat{p}}).
$), we need to solve the following set of functions to obtain $\varphi(\cdot)$ (short-handing $\varphi\circ s_{x}(\mathbf{\hat{p}})$ as $\varphi_x(\mathbf{\hat{p}})$):
\begin{align*}
s_0(\mathbf{\hat{p}})& = c_{0,0} \cdot \varphi_0(\mathbf{\hat{p}}) + c_{0,1}  \cdot \varphi_1(\mathbf{\hat{p}}) + \dots +c_{0,M-1}  \cdot \varphi_{M-1}(\mathbf{\hat{p}})\\
s_1(\mathbf{\hat{p}}) &= c_{1,0}  \cdot \varphi_0(\mathbf{\hat{p}}) + c_{1,1}  \cdot \varphi_1(\mathbf{\hat{p}}) + \dots +c_{1,M-1}  \cdot \varphi_{M-1}(\mathbf{\hat{p}})\\
&....\\
s_{M-1}(\mathbf{\hat{p}})& = c_{M-1,0}  \cdot \varphi_0(\mathbf{\hat{p}}) + c_{M-1,1}  \cdot \varphi_1(\mathbf{\hat{p}}) + \dots +c_{M-1,M-1}  \cdot \varphi_{M-1}(\mathbf{\hat{p}})
\end{align*}
Denote by $\mathbf{s}(\mathbf{\hat{p}}) = [s_0(\mathbf{\hat{p}});s_1(\mathbf{\hat{p}});...;s_{M-1}(\mathbf{\hat{p}})]$, and $\mathbf{\varphi}(\mathbf{\hat{p}}) = [\varphi_0(\mathbf{\hat{p}});\varphi_1(\mathbf{\hat{p}});...;\varphi_{M-1}(\mathbf{\hat{p}})]$. Then the above equation becomes equivalent with the following system of equation:
$\mathbf{s}(\mathbf{\hat{p}})  = C \cdot \mathbf{\varphi}(\mathbf{\hat{p}}). 
$ Choose a $C$ with full rank. For instance when $M>2$ we can set $\forall j$,
$
c_{j,j} = \frac{1}{2},~ c_{j,k} = \frac{1}{2(M-1)}, ~k \neq j
$ - not hard to verify that such a $C$ is indeed full rank. Then we are ready to solve for $\mathbf{\varphi}(\mathbf{p})$ as follows:
\begin{align}
\mathbf{\varphi}(\mathbf{\hat{p}}) = C^{-1}\cdot \mathbf{s}(\mathbf{\hat{p}}). \label{unbias:multi}
\end{align}
With defining above unbiased surrogate operator, all other discussions generalize fairly straight-forwardly - such a $\varphi$ will give us the same equation as established in the lemma below for the non-binary event outcome setting:
\begin{lemma}
Define $\varphi(\cdot)$ as in Eqn. (\ref{unbias:multi}), and flip $\tilde{X}_i$ using $C,x$. Then $\mathbb E_{\tilde{X}_i|x}[\varphi \circ s_{\tilde{X}_i=\tilde{x}_i}(\mathbf{\hat{p}})] = s_{x}(\mathbf{\hat{p}}).
$
\end{lemma}
We include a detailed example of $\varphi$ for three-outcome events below.
%\subsubsection{Different choice of $C$}
%There are clearly different ways of flipping the outcome, i.e., setting the $C$, while satisfying the full rank requirement. Through simulations (in Section XXX), we find that we have more risk for the $C$ that has smaller second-largest eigenvalue. How to theoretically argue above property remains an interesting theoretical question. 
%


\paragraph{Example of $\varphi$ for three-outcome events}

\begin{example}
An example with $M=3$. Suppose we flip the outcome using the uniform-error confusion matrix:
\[ C = 
\begin{bmatrix}
    0.5      & 0.25 &  0.25 \\
    0.25       & 0.5  & 0.25 \\
    0.25       & 0.25  & 0.5 
\end{bmatrix} \Rightarrow C^{-1} = 
\begin{bmatrix}
   3     & -1 &  -1 \\
    -1       & 3  & -1 \\
    -1       & -1  & 3 
\end{bmatrix}
\]
Therefore we obtain a closed-form of $\varphi$:
\begin{align*}
\mathbf{\varphi}_0 (\mathbf{\hat{p}})&= 3  \mathbf{s}_0(\mathbf{\hat{p}}) - \mathbf{s}_1(\mathbf{\hat{p}}) - \mathbf{s}_2(\mathbf{\hat{p}}) \\ 
\mathbf{\varphi}_1(\mathbf{\hat{p}}) &= - \mathbf{s}_0(\mathbf{\hat{p}}) +3 \mathbf{s}_1(\mathbf{\hat{p}}) - \mathbf{s}_2(\mathbf{\hat{p}}) \\ 
\mathbf{\varphi}_2(\mathbf{\hat{p}}) &= -  \mathbf{s}_0(\mathbf{\hat{p}}) - \mathbf{s}_1(\mathbf{\hat{p}}) + 3\mathbf{s}_2(\mathbf{\hat{p}}) 
\end{align*}
\end{example}



\section{Experimental evaluations}
In this section, we evaluate \textsf{LWS} and \textsf{LWS} with extensive simulations. We first compare the efficiency of \textsf{LWS} and \textsf{LWS} with that of other existing deterministic (weakly) incentive compatible mechanisms \textsf{WSWM}, \textsf{NAWM} and \textsf{DCA}. The results show that the two randomized wagering mechanisms outperform the three deterministic wagering mechanism. Then, we compare the variance of payoff and the probability of winning money within the two randomized wagering mechanisms. The results show that \textsf{RP-SWME} is better than \textsf{LWS} in these two matrices. 

\subsection{Simulation Setup}
We simulate both the binary events and the multi-outcome events.
For binary events, we generated six sets of agents' predictions and wagers according to the combinations of three different prediction models and two different wager models. With a little abuse of notation, we denote that an event happens with probability $q$ and that agent $i$ believes that the event to predict will happen with  probability $p_i$ and will not happen with probability $1-p_i$. We use three models to generate predictions $p_i,i\in\mathcal{N}$:
\begin{enumerate}
\item Uniform model: For each event, $p_i$ is independently drawn from a uniform distribution over $[0,1]$.
\item Logit-Normal model:  This model assumes that $p_i$, when being mapped to the real line by a logit function as $\log\left(\frac{p_i}{1-p_i}\right)$, is independently drawn from a Normal distribution $\mathcal{N}(\log(\frac{q}{1-q})^{1/\alpha}, \sigma^2)$, i.e., $p_i\sim \text{Logit-Normal}\left(\log(\frac{q}{1-q})^{1/\alpha}, \sigma^2\right)$.  $q, \alpha, \sigma^2$ are model parameters. This model is proposed and used to estimate the  happening probability of the event in~\cite{satopaa2014combining}, where $q$ is regarded as an estimator of the happening probability and $\alpha$ models the under-confident effect on human forecasters. Based on a real prediction dataset over 1300 forecasters and 69 geopolitical events collected in~\cite{satopaa2014combining}, this model outperforms most existing models to estimate the happening probability of events, which leads us to believe this model a good alternate to generate prediction data. In our simulations, we adopted $\alpha = 2$, which best fits the aforementioned real prediction dataset, $\sigma^2=1$, and $q$ is drawn uniformly from $[0,1]$ for each event. 

%of each agent is independently drawn from a Normal distribution when the prediction is mwith the This probability model relates the agents' probability predictions with the true probability of the event to predict. It is proposed in~\cite{satopaa2014combining} to infer  the true probability of the target event from agents' reported predictions and achieved best inference accuracy than existing models investigated~\cite{satopaa2014combining}. ....
\item Synthetic model: this synthetic model is introduced from a set of simulation studies in \cite{ranjan2010combining,allard2012probability,satopaa2014combining}. %\red{``This model  is an extension of the simulation study introduced by~\cite{ranjan2010combining} and further applied by~\cite{allard2012probability} and ~\cite{satopaa2014combining}''} 
 The model assumes that the happening probability of an event to be predicted by  $N$  is given by $q = \Phi(\sum_{i=1}^N u_i )$, where $\Phi$ is the cumulative distribution function of a standard normal distribution and $u_i$ is independently drawn from $\mathcal{N}(0,1)$. Each agent knows the true probability generating model and $u_i$ but not $u_j, \forall j\ne i$. Accordingly, each agent's calibrated belief of the happening probability of the event is given by $p_i = \Phi(\frac{u_i}{\sqrt{2N-1}})$.
\end{enumerate}

We use two models to generate the wagers of agents: 
 \begin{enumerate}
\item Uniform model: All agents' wagers are equal to 1.
\item Pareto model:  This model assumes that the wager $w_i$ of agent $i$ follows  the Pareto distribution, which is often adopted to model the distribution of wealth in a population. In the simulations of \cite{freeman2017double}, the authors selected the shape parameter and scale parameter of the Pareto distribution as 1.16 and 1 correspondingly, which is the distribution depicted as  ``20\% of the population has 80\% of the wealth''. We adopted the same parameters for comparison purpose. 
\end{enumerate}


For events with multiple outcomes, we simulated three sets of data with the number of possible outcomes 3, 6, 9 correspondingly. In each set, we drew the predictions from uniform distribution over the whole probability space and drew the wagers according to the Uniform model. 


\subsection{Comparison of efficiency of wagering mechanisms}

\begin{figure}[t]
\centering
\begin{subfigure}{0.28\textwidth}
\includegraphics[width=\textwidth]{0209risk_w_uniform_p_uniform.eps}
\caption{\label{risk_u_u}$\mathbf{p}\sim$ Uniform, $\mathbf{w}\sim$ Uniform}
\end{subfigure}\hspace{0.04\textwidth}
\begin{subfigure}{0.28\textwidth}
\includegraphics[width=\textwidth]{0209risk_w_uniform_p_logit.eps}
\caption{\label{risk_u_l}$\mathbf{p}\sim$ Logit, $\mathbf{w}\sim$ Uniform}
\end{subfigure}\hspace{0.04\textwidth}
\begin{subfigure}{0.28\textwidth}
\includegraphics[width=\textwidth]{0209risk_w_uniform_p_synthetic.eps}
\caption{\label{risk_u_s}$\mathbf{p}\sim$ Synthetic, $\mathbf{w}\sim$ Uniform}
\end{subfigure}
\begin{subfigure}{0.28\textwidth}
\includegraphics[width=\textwidth]{0209risk_w_pareto_p_uniform.eps}
\caption{$\mathbf{p}\sim$ Uniform, $\mathbf{w}\sim$ Pareto}
\label{risk_p_u}
\end{subfigure}\hspace{0.04\textwidth}
\begin{subfigure}{0.28\textwidth}
\includegraphics[width=\textwidth]{0209risk_w_pareto_p_logit.eps}
\caption{$\mathbf{p}\sim$ Logit, $\mathbf{w}\sim$ Pareto}
\label{risk_p_l}
\end{subfigure}\hspace{0.04\textwidth}
\begin{subfigure}{0.28\textwidth}
\includegraphics[width=\textwidth]{0209risk_w_pareto_p_synthetic.eps}
\caption{$\mathbf{p}\sim$ Synthetic, $\mathbf{w}\sim$ Pareto}
\label{risk_p_s}
\end{subfigure}
\caption{\label{risk_all}Average individual risk of each of five wagering mechanisms as a function of $N$ under different prediction and wager models}
\end{figure}
\begin{figure}[t]
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{risk_multi_3_w_uniform_p_uniform.eps}
\caption{\label{risk_multi_3}Events with 3 possible outcomes}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{risk_multi_6_w_uniform_p_uniform.eps}
\caption{\label{risk_multi_6}Events with 6 possible outcomes}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{risk_multi_9_w_uniform_p_uniform.eps}
\caption{\label{risk_multi_9}Events with 9 possible outcomes}
\end{subfigure}
\caption{\label{risk_multi_all}Average individual risk of each of four mechanisms under events with multiple outcomes}
\end{figure}
We show that \textsf{LWS} and  \textsf{RP-SWME} are more efficient than existing deterministic (weakly) incentive compatible mechanisms \textsf{WSWM}, \textsf{NAWM} and \textsf{DCA}. We evaluate the efficiency by two metrics: \emph{Average individual risk} and \emph{Average money exchange rate}.

\emph{Individual risk} is the percent of wager that an individual agent can lose in the worst case w.r.t. the event outcome and the randomness of the mechanisms. The average individual risk is an indicator of Pareto optimality, because the average individual risk equal to 1 (i.e., no one can commit to secure a positive wager before the wagering game) is a sufficient condition of Pareto optimality.
%The closer to 1 the risk is, the less available wager the agent has to make a side bet with. 
\emph{Money exchange rate} is the total amount of money exchanged  in the game after the outcome of a wagering mechanism is realized, divided by the total amount of wagers. Average money exchange rate measures the efficiency of an average wagering game.  


In our simulations, we vary the number of agents for 2 to 50 with a step of 2. For each number of agents, we randomly generate 1000 events and the agents' predictions and wagers for each of the six combinations of prediction models and wager models, and take the average of individual risk  and money exchange rate over the 1000 events. When calculating the money exchange, we use the expectation of the money exchange over all possible outcomes according to the happening probability of each outcome. This happening probability is either specified in the model generating the predictions, or otherwise, drawn from a uniform distribution over the corresponding probability space. 

In the simulations, both \textsf{RP-SWME} and \textsf{LWS} achieve the highest average individual risk (approximately 1)  under all conditions (\# of outcomes, \# of agents, prediction models, and wager models) we simulated (Figure~\ref{risk_all}, \ref{risk_multi_all}). %\footnote{The simulation results on events with multiple outcomes, i.e., Figure~\ref{risk_multi_all}, is presented in Appendix}. 
In contrast, the best of the deterministic mechanisms \textsf{DCA}, only achieves an approximate 1 average individual risk  when the wagers of agents are uniform and the number of participants is more than 30 (Figure~\ref{risk_u_u}-\ref{risk_u_s}). Its average individual risk drops to 0.6 when the wagers of agents follows the Pareto distribution (Figure~\ref{risk_p_u}-\ref{risk_p_s}). This result shows that the two randomized mechanisms effectively remove the opportunity for side bet and take use of all the wagers before the outcome is realized. %We have similar observations for money exchange rate. %and defer the detailed results to Appendix due to space limit.


\textsf{LWS}  doubles the money exchange rate of the second best alternative, hitting a more than 80\% money exchange rate under all conditions we simulated (Figure~\ref{me_all}, \ref{me_multi_all}). On the other hand, \textsf{RP-SWME} also defeats the other two incentive compatible deterministic wagering mechanisms in expected money exchange under all conditions we simulated  (Figure~\ref{me_all}, \ref{me_multi_all}). Meanwhile, it also outperforms \textsf{DCA} when the number of agents is small  (Figure~\ref{me_all}).

In particular, when the prediction follows the synthetic model, where the predictions are much closer to each other as  the number of participants increases,  the money exchange rate of the two incentive compatible deterministic wagering mechanisms,  \textsf{WSWM} and  \textsf{NAWM}  converge to zero. However, the two randomized wagering mechanisms still keep a large money exchange rate (Figure~\ref{me_u_s}, \ref{me_p_s}).

\begin{figure}[t]
\centering
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{0209me_w_uniform_p_uniform.eps}
\caption{$\mathbf{p}\sim$ Uniform, $\mathbf{w}\sim$ Uniform}
\label{me_u_u}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{0209me_w_uniform_p_logit.eps}
\caption{$\mathbf{p}\sim$ Logit, $\mathbf{w}\sim$ Uniform}
\label{me_u_l}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{0209me_w_uniform_p_synthetic.eps}
\caption{$\mathbf{p}\sim$ Synthetic, $\mathbf{w}\sim$ Uniform}
\label{me_u_s}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{0209me_w_pareto_p_uniform.eps}
\caption{$\mathbf{p}\sim$ Uniform, $\mathbf{w}\sim$ Pareto}
\label{me_p_u}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{0209me_w_pareto_p_logit.eps}
\caption{$\mathbf{p}\sim$ Logit, $\mathbf{w}\sim$ Pareto}
\label{me_p_l}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{0209me_w_pareto_p_synthetic.eps}
\caption{$\mathbf{p}\sim$ Synthetic, $\mathbf{w}\sim$ Pareto}
\label{me_p_s}
\end{subfigure}
\caption{\label{me_all}Average money exchange rate of each of five wagering mechanisms as a function of $N$ under different prediction and wager models}
\end{figure}


\begin{figure}[h]
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{me_multi_3_w_uniform_p_uniform.eps}
\caption{\label{me_multi_3}Events with 3 possible outcomes}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{me_multi_6_w_uniform_p_uniform.eps}
\caption{\label{me_multi_6}Events with 6 possible outcomes}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{me_multi_9_w_uniform_p_uniform.eps}
\caption{\label{me_multi_9}Events with 9 possible outcomes}
\end{subfigure}
\caption{\label{me_multi_all}Average money exchange rate of each of four mechanisms under events with multiple outcomes}
\end{figure}


\subsection{Comparison of randomness properties of  \textsf{RP-SWME} and  \textsf{LWS}}
\label{sim_var_pr}
In this section, we compare the \emph{standard variance} of payoffs and \emph{the probability of not losing money} of \textsf{RP-SWME} and \textsf{LWS}. We evaluated these two metrics w.r.t. to the prediction accuracy, which is measured based on the distance of a prediction to the outcome, i.e., $\text{Accuracy} = 1 - |x-p_i|$\footnote{We use it as measurement of accuracy for two reasons: i. it is linear in prediction $p_i$, ii. it has an inject to Brier Score}.


In the evaluation, we run 10000 wagering instances under these two mechanisms and recorded the prediction accuracy of each agent in each instance and the corresponding net-payoff. Then, we group these agents into 10 groups that correspond to 10 consecutive accuracy intervals. In each group, we calculate the standard variance and the percent of agents winning money. For fair comparison, we normalize the net-payoff of each agent by its own wager.

We simulate binary events. We generate two set of simulated data. In both sets, we varied the number of agents from 2 to 50 with a set of 2, and under each number, we generated 10000 instances. In each instance, the agents' predictions are drawn from the Uniform model, while the wagers are drawn from the Uniform model in one set and drawn from the Pareto model in the other set. 

Our results show that under all conditions we simulate, \textsf{RP-SWME} has a much smaller variance in agents' net-payoff and the variance is steady across agents with different prediction accuracy. In contrast, the \textsf{LWS} has a much larger variance in net-payoff, which increases with the prediction accuracy (Figure~\ref{std_all}). On the other hand,  \textsf{RP-SWME} has a much larger probability of not losing money and this probability increases with the prediction accuracy, while \textsf{LWS} has a much smaller such probability (Figure~\ref{pr_all}). In brief, while both \textsf{RP-SWME} and \textsf{LWS} can effectively improve the efficiency of wagering, \textsf{RP-SWME} provides much less uncertainty than \textsf{LWS} does and thus, may be regarded as a more attractive alternative for deterministic wagering mechanisms. 

\begin{figure}[!t]
\begin{minipage}{0.50\textwidth}
%\begin{subfigure}{0.24\textwidth}
%\includegraphics[width=\textwidth]{std_p_true_1_newrand_w_uniform_p_uniform.eps}
%\caption{\label{std_p_uniform} $accuracy = 1 - |q - p_i|$, $\mathbf{w}\sim$ Uniform}
%\end{subfigure}
\begin{subfigure}{0.46\textwidth}
\includegraphics[width=\textwidth]{std_outcome1_newrand_w_uniform_p_uniform.eps}
\caption{\label{std_o_uniform}
%$accuracy = 1 - |o - p_i|$, 
$\mathbf{w}\sim$ Uniform}
\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%\includegraphics[width=\textwidth]{std_p_true_1_newrand_w_pareto_p_uniform.eps}
%\caption{\label{std_p_pareto}$accuracy = 1 - |q - p_i|$, $\mathbf{w}\sim$ Pareto}
%\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\textwidth]{std_outcome1_newrand_w_pareto_p_uniform.eps}
\caption{\label{std_o_pareto}
%$accuracy = 1 - |o - p_i|$, 
$\mathbf{w}\sim$ Pareto}
\end{subfigure}
\caption{\label{std_all}Std. variance of net-payoff as a function of prediction accuracy: \textsf{RP-SWME} v.s. \textsf{LWS}}
%\vspace{-0.5em}
\end{minipage}
\begin{minipage}{0.50\textwidth}
%\begin{subfigure}{0.24\textwidth}
%\includegraphics[width=\textwidth]{pr_p_true_1_newrand_w_uniform_p_uniform.eps}
%\caption{\label{pr_p_uniform}$accuracy = 1 - |q - p_i|$, $\mathbf{w}\sim$ Uniform}
%\end{subfigure}
\begin{subfigure}{0.46\textwidth}
\includegraphics[width=\textwidth]{pr_outcome1_newrand_w_uniform_p_uniform.eps}
\caption{\label{pr_o_uniform}
%$accuracy = 1 - |o - p_i|$, 
$\mathbf{w}\sim$ Uniform}
\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%\includegraphics[width=\textwidth]{pr_p_true_1_newrand_w_pareto_p_uniform.eps}
%\caption{\label{pr_p_pareto}$accuracy = 1 - |q - p_i|$, $\mathbf{w}\sim$ Pareto}
%\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\textwidth]{pr_outcome1_newrand_w_pareto_p_uniform.eps}
\caption{\label{pr_o_pareto}
%$accuracy = 1 - |o - p_i|$, 
$\mathbf{w}\sim$ Pareto}
\end{subfigure}
\caption{\label{pr_all}Probability of not losing money as a function of prediction accuracy: \textsf{RP-SWME} v.s. \textsf{LWS}}
\end{minipage}
\end{figure}



%We define the following two metrics to further evaluate randomized wagering mechanisms,  the \emph{variance of payoff} and the \emph{probability of winning money}.
%\begin{definition}[Variance of Payoff]
%Given $\report{}, \mathbf{w}, x$, the \emph{variance} of payoff for agent $i$ under a randomized wagering mechanism is defined as follows: $$\mathbb{E}_{\mathcal{D}(\report{}, \mathbf{w}, x)}\left[\left(\Pi_i(\report{}, \mathbf{w}, x) - \mathbb{E}_{\mathcal{D}(\report{}, \mathbf{w}, x)}[\Pi_i(\report{}, \mathbf{w}, x)\right)^2]\right].$$
%\end{definition}
%\begin{definition}[Chance of Winning]
%Given $\report{}, \mathbf{w}, x$, the \emph{probability of winning money} for agent $i$ under a randomized wagering mechanism is defined as follows: 
%$$
%\int_{0}^{+\infty}\int_{\mathbb{R}^{N-1}}f_i^{\mathcal{D}(\report{}, \mathbf{w}, x)}(\pi_i,\mathbf{\pi}_{-i})d\mathbf{\pi}_{-i}d\pi_i.
%$$
%\end{definition}






%\comy{this can go to appendix}

==> experiment_full_version.tex <==
\section{Simulations}\label{sec:simulation}
%The (weakly) incentive compatible deterministic wagering mechanisms always suffer from low efficiency (low risk and low money exchange) in the sense that agents can win or lose by only a limited amount of money w.r.t. the wagers they put in. In contrast, as we show in our theoretical analysis, randomized wagering mechanism can overcome this problem by properly transferring the payoff as a randomized variable. 
%In this section, we first compare the risk and money exchange of the \textsf{RP-SWS} and \textsf{LWS} with existing typical (weakly) incentive compatible deterministic wagering mechanisms in simulations, and show that both \textsf{RP-SWS} and \textsf{LWS} outperform these deterministic wagering mechanisms. 

%Second, in randomized wagering mechanisms,  as the payoffs of agents are random variables, expectation and standard variance are two natural metrics to evaluate with. We show with simulations that while the \textsf{RP-SWS} and \textsf{LWS} have the same expected payoff for each input profile (agents' prediction, wagers, outcomes), \textsf{RP-SWS} maintains a much smaller variance in agents' payoff. Furthermore, the probability of not losing money is also a critical metric, as human agents are always trying to avoid loss. From this perspective, we also show in simulations that participants in \textsf{RP-SWS} has a much higher probability of not losing money.  We believe that these two properties make the \textsf{RP-SWS} a more attractive alternative than the \textsf{LWS} to improve the wagering efficiency.

%Furthermore, the probability of not losing money is also critical, as avoiding loss is human nature.
\vspace{-0.5em}
\subsection{Efficiency comparison with deterministic wagering mechanisms}
\label{subsec_comp1}
We compare the \emph{individual risk} and the \emph{money exchange rate} of the Brier scoring rule based \textsf{RP-SWS}, \textsf{LWS} with the \textsf{DCA}, the Brier scoring rule based \textsf{WSWM} and the Brier scoring rule based \textsf{NAWM}, the three only other known, non-trivial wagering mechanisms that satisfy individually rational, (weakly) incentive compatible, (weakly) budget balance.

The \emph{individual risk} is the maximum percent of wager that an individual agent may lose in the game before the outcome of the wagering mechanism is realized. The closer to 1 the risk is, the less available wager the agent has to make a side bet with. The \emph{money exchange rate} is the total amount of money exchanged  in the game after the outcome of a wagering mechanism is realized, divided by the total amount of wagers.  These two metrics are natural metrics measuring the efficiency as they reflect to which degree the difference of agents' beliefs and wagers are transformed into money exchange in the worst case or in a specified case. 

We compare these two metrics under both events with binary outcomes and events with multiple outcomes. For events with binary outcomes, among the three deterministic mechanisms we compare with, the \textsf{DCA} has the highest individual risk and money exchange~\cite{freeman2017double}, thus, it serves as the baseline comparison. However, while our randomized wagering mechanisms satisfy the incentive compatibility, \textsf{DCA} only satisfies the weakly incentive compatibility. Therefore, we also include \textsf{WSWM} and \textsf{NAWM} to serve as the deterministic counterpart that also satisfy incentive compatibility. 
For events with multiple outcomes, where the \textsf{DCA} cannot be applied, we compare the \textsf{RP-SWS} and \textsf{LWS} with only the \textsf{WSWM} and the \textsf{NAWM}. 

%In our simulations, we show that the RP-SWM mechanism outperforms the \textsf{DCA} in individual risk as the average individual risk of the RP-SWM is approximately 1. Meanwhile, when the number of agents is small, the RP-SWM also achieves the much better money exchange rate than \textsf{DCA}. For events with multiple outcomes, where the \textsf{DCA} does not work, the RP-SWM also achieves approximately 1 average individual risk and much higher money exchange than the \textsf{WSWM} and the NAWM.

%
%\subsubsection{Results}
%\textbf{}

\paragraph{Results:} For detailed setting of our simulations, please refer to Appendix. In the simulations, both \textsf{RP-SWS} and \textsf{LWS} achieve the highest average individual risk (approximately 1)  under all conditions (\# of outcomes, \# of agents, prediction models, and wager models) we simulated (Figure~\ref{risk_all}, \ref{risk_multi_all})\footnote{The simulation results on events with multiple outcomes, i.e., Figure~\ref{risk_multi_all}, is presented in Appendix}. In contrast, the best of the deterministic mechanisms \textsf{DCA}, only achieves an approximate 1 average individual risk  when the wagers of agents are uniform and the number of participants is more than 30 (Figure~\ref{risk_u_u}-\ref{risk_u_s}). Its average individual risk drops to 0.6 when the wagers of agents follows the Pareto distribution (Figure~\ref{risk_p_u}-\ref{risk_p_s}). This result shows that the two randomized mechanisms effectively remove the opportunity for side bet and take use of all the wagers before the outcome is realized. We have similar observations for money exchange rate and defer the detailed results to Appendix due to space limit.

%
%\begin{figure}[t]
%\centering
%\begin{subfigure}{0.28\textwidth}
%\includegraphics[width=\textwidth]{0209risk_w_uniform_p_uniform.eps}
%\caption{\label{risk_u_u}$\mathbf{p}\sim$ Uniform, $\mathbf{w}\sim$ Uniform}
%\end{subfigure}\hspace{0.04\textwidth}
%\begin{subfigure}{0.28\textwidth}
%\includegraphics[width=\textwidth]{0209risk_w_uniform_p_logit.eps}
%\caption{\label{risk_u_l}$\mathbf{p}\sim$ Logit, $\mathbf{w}\sim$ Uniform}
%\end{subfigure}\hspace{0.04\textwidth}
%\begin{subfigure}{0.28\textwidth}
%\includegraphics[width=\textwidth]{0209risk_w_uniform_p_synthetic.eps}
%\caption{\label{risk_u_s}$\mathbf{p}\sim$ Synthetic, $\mathbf{w}\sim$ Uniform}
%\end{subfigure}
%
%\begin{subfigure}{0.28\textwidth}
%\includegraphics[width=\textwidth]{0209risk_w_pareto_p_uniform.eps}
%\caption{$\mathbf{p}\sim$ Uniform, $\mathbf{w}\sim$ Pareto}
%\label{risk_p_u}
%\end{subfigure}\hspace{0.04\textwidth}
%\begin{subfigure}{0.28\textwidth}
%\includegraphics[width=\textwidth]{0209risk_w_pareto_p_logit.eps}
%\caption{$\mathbf{p}\sim$ Logit, $\mathbf{w}\sim$ Pareto}
%\label{risk_p_l}
%\end{subfigure}\hspace{0.04\textwidth}
%\begin{subfigure}{0.28\textwidth}
%\includegraphics[width=\textwidth]{0209risk_w_pareto_p_synthetic.eps}
%\caption{$\mathbf{p}\sim$ Synthetic, $\mathbf{w}\sim$ Pareto}
%\label{risk_p_s}
%\end{subfigure}
%\caption{\label{risk_all}Average individual risk of each of five wagering mechanisms as a function of $N$ under different prediction and wager models}
%
%\end{figure}




\vspace{-0.5em}
\subsection{Comparison of randomness properties between the \textsf{RP-SWS} and the \textsf{LWS}}
\label{sim_var_pr}
In this section, we compare the \emph{standard variance} of payoffs and \emph{the probability of not losing money} of \textsf{RP-SWS} and \textsf{LWS}. We evaluated these two metrics w.r.t. to the prediction accuracy. In other words, we ran a larger number of wagering instances under these two mechanisms and recorded the prediction accuracy of each agent in each instance and the corresponding net-payoff. Then, we group these agents into 10 groups that correspond to 10 consecutive accuracy ranges. In each group, we calculated the standard variance and the percent of agents not losing money. For fair comparison, we normalized the net-payoff of each agent by its own wager.

We simulated events with binary outcome but we observe similar results for events with multiple outcomes. We generated two set of simulated data. In both sets, we varied the number of agents from 2 to 50 with a set of 2, and under each number, we generated 10000 instances. In each instance, the agents' predictions were drawn from the Uniform model, while the wagers were drawn from the Uniform model in one set and drawn from the Pareto model in the other set. Under each set of data, we measured  the prediction accuracy in two ways. For the first one, we used the distance of the agent's prediction and the true happening probability to  measure the accuracy, i.e., $accuracy = 1 - |q - p_i|$, where $q$ is the true happening probability of outcome 1, and the $p_i$ the happening probability of outcome 1 reported by agent $i$. In the second way, we used the distance of the agent's prediction and the true outcome to  measure the accuracy, i.e., $accuracy = 1 - |o - p_i|$, where $o=1$ if outcome 1 happens, otherwise $o=0$. 

Our results show that under all conditions we simulated, \textsf{RP-SWS} has a much smaller variance in agents' net-payoff and the variance is steady across agents with different prediction accuracy. In contrast, the \textsf{LWS} has a much larger variance in net-payoff, which increases with the prediction accuracy (Figure~\ref{std_all}). On the other hand,  \textsf{RP-SWS} has a much larger probability of not losing money and this probability increases with the prediction accuracy, while \textsf{LWS} has a much smaller such probability (Figure~\ref{pr_all}). In brief, while both \textsf{RP-SWS} and \textsf{LWS} can effectively improve the efficiency of wagering, \textsf{RP-SWS} provides much less uncertainty than \textsf{LWS} does and thus, may be regarded as a more attractive alternative for deterministic wagering mechanisms. 

%\begin{figure}[t]
%\begin{subfigure}{0.24\textwidth}
%\includegraphics[width=\textwidth]{std_p_true_1_newrand_w_uniform_p_uniform.eps}
%\caption{\label{std_p_uniform} $accuracy = 1 - |q - p_i|$, $\mathbf{w}\sim$ Uniform}
%\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%\includegraphics[width=\textwidth]{std_outcome1_newrand_w_uniform_p_uniform.eps}
%\caption{\label{std_o_uniform}$accuracy = 1 - |o - p_i|$, $\mathbf{w}\sim$ Uniform }
%\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%\includegraphics[width=\textwidth]{std_p_true_1_newrand_w_pareto_p_uniform.eps}
%\caption{\label{std_p_pareto}$accuracy = 1 - |q - p_i|$, $\mathbf{w}\sim$ Pareto}
%\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%\includegraphics[width=\textwidth]{std_outcome1_newrand_w_pareto_p_uniform.eps}
%\caption{\label{std_o_pareto}$accuracy = 1 - |o - p_i|$, $\mathbf{w}\sim$ Pareto}
%\end{subfigure}
%\caption{\label{std_all}Std. variance of net-payoff as a function of prediction accuracy: \textsf{RP-SWS} v.s. \textsf{LWS}}
%\vspace{-0.5em}
%\end{figure}
%\vspace{-0.5em}
%\begin{figure}[t]
%\begin{subfigure}{0.24\textwidth}
%\includegraphics[width=\textwidth]{pr_p_true_1_newrand_w_uniform_p_uniform.eps}
%\caption{\label{pr_p_uniform}$accuracy = 1 - |q - p_i|$, $\mathbf{w}\sim$ Uniform}
%\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%\includegraphics[width=\textwidth]{pr_outcome1_newrand_w_uniform_p_uniform.eps}
%\caption{\label{pr_o_uniform}$accuracy = 1 - |o - p_i|$, $\mathbf{w}\sim$ Uniform}
%\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%\includegraphics[width=\textwidth]{pr_p_true_1_newrand_w_pareto_p_uniform.eps}
%\caption{\label{pr_p_pareto}$accuracy = 1 - |q - p_i|$, $\mathbf{w}\sim$ Pareto}
%\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%\includegraphics[width=\textwidth]{pr_outcome1_newrand_w_pareto_p_uniform.eps}
%\caption{\label{pr_o_pareto}$accuracy = 1 - |o - p_i|$, $\mathbf{w}\sim$ Pareto}
%\end{subfigure}
%\caption{\label{pr_all}Probability of not losing money as a function of prediction accuracy: \textsf{RP-SWS} v.s. \textsf{LWS}}
%\end{figure}

==> pareto.tex <==
%\subsection{Money exchange/risk property}


%\begin{align*}
%&(\frac{1-e_1}{1-e_1-e_0} + \frac{e_0}{1-e_1-e_0} + \frac{2e_1}{1-e_1-e_0})\cdot \frac{1}{1+\frac{2e_1}{1-e_1-e_0}} = \frac{1+e_0+e_1}{1-e_0+e_1}\\
%&(\frac{1-e_1}{1-e_1-e_0} + \frac{e_0}{1-e_1-e_0}+\frac{2e_0}{1-e_1-e_0})\cdot \frac{1}{1+\frac{2e_0}{1-e_1-e_0}} = \frac{1+3e_0-e_1}{1-e_1+e_0}
%\end{align*}
%again each agent can win as much as 150\% of his wager when we set  $e_0 = e_1 = 0.25$. 

%\begin{proposition}
%The impossibility results for Pareto optimality condition holds for randomized wagering mechanism w.r.t. expected utility. 
%\end{proposition}

\subsection{Pareto optimality}

Bringing in this additional layer of randomness turns out to benefit us with good Pareto efficiency properties. In general, adding randomness will help add more variance of agents' payoffs, pushing the mechanism to Pareto optimality. However directly adding random noises will (1) decrease the incentive levels and (2) violate the established properties of the deterministic wagering mechanisms. Our method provides a way for intervening with randomness but then removing the introduced bias in expectation. In a nutshell, we provide another level of `gambling' that when an agent's reported belief predicts his surrogate outcome well, he will be rewarded even more; but on the other hand, he may risk losing more due to the random flipping nature of the surrogate outcomes. This will significantly increase the Pareto efficiency of each participant's wagers - but in expectation the above two effects will cancel out so agents' incentives in truthful reporting would not change. 

%To see this intuitively, for instance, when the true outcome is 1, the most scaled possible payment is at least $\frac{1-e_0}{1-e_1-e_0}$ (happens when the surrogate outcome for a particular agent stays to be the same as the true outcome). For instance when we set the flipping probabilities to be $e_0 = e_1 = 0.3$. We will have $\frac{1-e_0}{1-e_0-e_1} = \frac{7}{4},$
%that is each agent can indeed win as much as 175\% as he originally can make. Similarly as other agent's surrogate scores can be scaled up by $\frac{1-e_0}{1-e_0-e_1}$, each agent also risks losing up to $175\%$ of what he was originally losing. We will provide extensive experimental results to validate above claim.



\begin{theorem}
(\textsf{RP-SWS}) satisfies Pareto-optimality.
\end{theorem}
\begin{proof}

\end{proof}


%\com{TODO: Cite pareto optimality, and mention risk properties}
%
%\com{define parato optimality}
%
%\com{summarize a list of risk properties that we would like to test}
%
%We define a list of properties that captures risk and potential:
%\begin{itemize}
%\item worst/expected case money loss (for each agent)
%\item best/expected case money gain
%\end{itemize}




==> property.tex <==
\subsection{Proof of Theorem~2
%\ref{thm:sws}
}\label{sec:proof}

%We show that the surrogate wagering mechanism (SWM) defined over WSWM satisfies all properties (a)-(i), and invokes larger money exchange and agents face possibly much higher return from wagering.
\begin{proof}


\underline{(a) Individual rationality:} This follows immediately from the results for \textsf{WSWM}, in light of the unbiasedness proof for surrogate \textsf{WSWM}. %(Eqn.(\ref{unbias:sws})).

~\\

\underline{(b) Strictly Incentive Compatibility:} 
First consider \textsf{SWME}. For an arbitrary profile of reports $\hp$ and wagers $\bw$, Algorithm~3 outputs an profile $\mathcal E$ of error rates of all agents. %Consider agent $i$, and an arbitrary set of reported predictions from agents - denote this event by $\mathcal E$, and 
Denote by $\hat{\varphi}^i_{\mathcal E}(\cdot)$ the corresponding surrogate function specified using the error rate profile $\mathcal E$ for agent $i$. For each $i$ and $j \in \mathcal N$:
\begin{align*}
&\mathbb E_{X\sim p_i,\tilde{X}_j}\bigl [\hat{\varphi}^j_{\mathcal E} \circ  s_{\tilde{X}_j}(\hat{p}_j)\bigr] = p_i \mathbb E_{\tilde{X}_j|X=1}[\hat{\varphi}^j_{\mathcal E} \circ s_{\tilde{X}_j}
(\hat{p}_j)]\\
+&(1-p_i) \mathbb E_{\tilde{X}_j|X=0}[\hat{\varphi}^j_{\mathcal E} \circ s_{\tilde{X}_j}(\hat{p}_j)]\\
=&p_i \cdot s_{X = 1}
(\hat{p}_j) + (1-p_i)\cdot s_{X = 0}
(\hat{p}_j) = \mathbb E_{X\sim p_i}[s_{X}(\hat{p}_j)],
\end{align*}
using Corollary~1. Then (using linearity of expectation, note $\tilde{\mathbf{X}}$ encode the randomness in $\Pi^{\textsf{SWME}}_i$)
%$\Pi^{\text{SWME}}_i$ is defined using $\hat{\varphi}_{\mathcal E_i}(\cdot)$:
\begin{align*}
&\mathbb E_{X\sim p_i,\tilde{\mathbf{X}}}\bigl[\Pi^{\textsf{SWME}}_i(\hp,\mathbf{w},X)\bigr]\\ %:= \varphi \circ \Pi^{\text{\emph{WS}}}_i(p_i,\mathbf{p}_{-i},\mathbf{w},\outcome{}) \nonumber \\
=& \frac{w_i W_{\mathcal{N}\backslash \{i\}}}{W_{\mathcal{N}}}\biggl( \mathbb E_{X\sim p_i,\tilde{X}_i}[\hat{\varphi}^i_{\mathcal E} \circ s_{\tilde{X}_i}(\hat{p}_i)] \nonumber \\
-& \sum_{j \in \mathcal{N}\backslash \{i\}} \frac{w_j}{W_{\mathcal{N}\backslash \{i\}}} \mathbb E_{X\sim p_i,\tilde{X}_j}[\hat{\varphi}^j_{\mathcal E} \circ s_{\tilde{X}_j}(\hat{p}_j)]\biggr)\\
=& \mathbb E_{X\sim p_i}\biggl[\frac{w_i W_{\mathcal{N}\backslash \{i\}}}{W_{\mathcal{N}}}\biggl( s_{X}(\hat{p}_i) - \sum_{j \in \mathcal{N}\backslash \{i\}} \frac{w_j}{W_{\mathcal{N}\backslash \{i\}}}  s_{X}(\hat{p}_j)\biggr)\biggr]\\
=&\mathbb E_{X\sim p_i}\bigl[ \Pi^{\text{WS}}_i(\hp,\mathbf{w},X) \bigr]~.
\end{align*}

Note the above holds for any possible reports ($\forall \mathcal E$). Thus the incentive properties of \textsf{WSWM} will preserve, i.e., reporting truthfully agent $i$'s private belief returns a higher payoff. The proof for  \textsf{RP-SWME} is similar, with the only difference in that each agent's net-payoff is further averaged over the random partitions (but SIC under each possible partition). 

~\\

\underline{(c) Budget Balance:} For (\textsf{SWME}), it suffices to prove $\sum_i \Pi^{\text{SWME}}_i(\hat{p}_i, w_i, \cdot) = 0.$ This can be easily proved by writing down the sum of $\Pi^{\text{SWME}}_i(\hat{p}_i, w_i, \cdot)$s. 
\begin{align*}
\sum_i \Pi^{\text{SWME}}_i(\hat{p}_i, w_i, \cdot) =& \sum_i \frac{w_i W_{\mathcal N\backslash \{i\}}}{W_{\mathcal N}}\biggl( \varphi \circ s_{\tilde{x}_i}(\hat{p}_i) - \sum_{j \in \mathcal N\backslash \{i\}} \frac{w_j}{W_{\mathcal N\backslash \{i\}}}{W_{\mathcal N}} \cdot \varphi \circ s_{\tilde{x}_j}(\hat{p}_j)\biggr)\\
=&\sum_i \biggl( \frac{w_i W_{\mathcal N\backslash \{i\}}}{W_{\mathcal N}} \varphi \circ s_{\tilde{x}_i}(\hat{p}_i)  - \sum_{j \neq i} \frac{w_j W_{\mathcal N\backslash \{j\}}}{W_{\mathcal N}} \cdot  \frac{w_i}{W_{\mathcal N \backslash \{j\}}}{W_{\mathcal N}} \cdot \varphi \circ s_{\tilde{x}_i}(\hat{p}_i) \biggr)\\
=&\sum_i \biggl( \frac{w_i W_{\mathcal N\backslash \{i\}}}{W_{\mathcal N}} \varphi \circ s_{\tilde{x}_i}(\hat{p}_i)  - \frac{w_i W_{\mathcal N\backslash \{i\}}}{W_{\mathcal N}} \varphi \circ s_{\tilde{x}_i}(\hat{p}_i) \biggr) = 0.
\end{align*}
%\com{to be added.}

The above also shows that for each group from the random partition of (\textsf{RP-SWME}), budget balance is satisfied. Thus we also proved budget balance for (\textsf{RP-SWME}).

~\\ 

\underline{(d) Sybilproofness:} \textsf{SWME} is sybilproof as we proved that the expected payoffs of \textsf{SWME} are the same as \textsf{WSWM} (and \textsf{WSWM} is Sybilproof). \textsf{RP-SWME} is also Sybilproof as a corollary of the following lemma.
%~\ref{LM:SYB}
%The proof of the lemma is presented in the Appendix.
\begin{lemma}
\label{LM:SYB}
If a (randomized) wagering mechanism $\mathcal W$ is (weakly) budget-balanced, (weakly) incentive compatible, Sybilproof, then the mechanism $\mathcal W*$ that first uniformly randomly pairs agents in groups of two and then runs mechanism $\mathcal W$ for each group is still Sybilproof.
\end{lemma} 


\begin{proof}
We prove the claim for the case that an agent is only allowed to create two identities. The claim holds in general, as we can alway merge two identities into one without decreasing the payoff, following the result of the case of two. 

Fixing an arbitrary belief $\mathbf{p}_i$ of agent $i$, we denote the $E_i^{\mathcal W}(\report{},\mathbf{w}):=\mathbb{E}_{X\sim\mathbf{p}_i, \mathcal{D}^{\mathcal W}(\report{},\mathbf{w},X)}[\Pi_i(\report{},\mathbf{w},X=x)] $, where $\mathcal{D}^{\mathcal W}(\cdot)$ is the distribution specified by mechanism $\mathcal W$. 
Suppose an agent $i$ divides its wager $w_i$ into two wagers   $w_{i1}, w_{i2}$, and reports two predictions $\report{i1}, \report{i2}$ correspondingly. 
We have $\forall \report{i1}, \report{i2}, w_{i1}, w_{i2}, \report{-i}, \mathbf{w}_{-i}, x$, 
\begin{small}
\begin{align*}
& E_i^{\mathcal W*}(\report{i1}, \report{i2},  \report{-i}, w_{i1}, w_{i2}, \mathbf{w}_{-i})  \\
=  &  \sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\report{i1}, \report{j}, w_{i1}, w_j) +\sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\report{i2}, \report{j}, w_{i2}, w_j) 
+
 \frac{1}{N}\left(E_{i1}^{\mathcal W}(\report{i1}, \report{i2}, w_{i1}, w_{i2}) + E_{i2}^{\mathcal W}(\report{i1},\report{i2},w_{i1}, w_{i2})\right) \\
\le & \sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\report{i1}, \report{j}, w_{i1}, w_j) +\sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\report{i2}, \report{j}, w_{i2}, w_j) 
\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, 
(\mathcal W\text{ is (weakly) budget balance})\\
\le & \sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\mathbf{p}_i, \report{j}, w_{i1}, w_j) +\sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\mathbf{p}_i, \report{j}, w_{i2}, w_j) 
\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,
 (\mathcal W\text{ is (weakly) incentive compatible})\\
\le & \sum_{j\ne i} \frac{1}{N}E_i^{\mathcal W}(\mathbf{p}_i, \report{j}, w_{i}, w_j) 
\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, \,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, 
\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,
 (\mathcal W\text{ is sybilproof})\\
\le &  \sum_{j\ne i} \frac{1}{N-1}E_i^{\mathcal W}(\mathbf{p}_i, \report{j}, w_{i}, w_j) =  E_i^{\mathcal W*}(\mathbf{p}_i, \report{-i}, w_{i}, \mathbf{w}_{-i})
\end{align*}
\end{small}
Therefore,  $\mathcal W*$ is sybilproof.
\end{proof}

~\\

\underline{(d) Anonymity:} For \textsf{SWME}, this proof can follow from the fact that the randomness (error rate selection) in \textsf{SWME} and t\textsf{RP-SWME} depends only on the reports and wagers of agents and do not depend on the identities of agents and the fact that the expected net-payoffs of agents are the same with those of \textsf{WSWM} (Corollary 1), which is anonymous~\cite{lambert2008self}. \textsf{RP-SWME} only adds a random partition of agents in \textsf{SWME} and the partition does not depend on the identities of agents. Thus, \textsf{RP-SWME} is also anonymous.
~\\

\underline{(f) Neutrality:} For \textsf{SWME}, this proof can follow from the fact that the randomness (error rate selection) in \textsf{SWME} and t\textsf{RP-SWME} depends only on the reports and wagers of agents and do not depend on the labeling of the outcomes and the fact that the expected net-payoffs of agents are the same with those of \textsf{WSWM} (Corollary 1), which is neutral~\cite{lambert2008self}. \textsf{RP-SWME} only adds a random partition of agents in \textsf{SWME} and the partition does not depend on the labeling of the outcomes. Thus, \textsf{RP-SWME} is also neutral.

~\\

\underline{(g) Non-arbitrage opportunity:} Now we prove that \textsf{SWME} does not allow arbitrage opportunity. The idea is simple and straight-forward: fix the set of prediction $\mathbf{p}_{-i}$ and wagers $\mathbf{w}$. First notice the fact that under each possible realization $\tilde{x}_i$, $\tilde{x}_{-i}$ can be any possible realizations. Since $s_{\tilde{X}_i=1}(p_i)$ and $s_{\tilde{X}_i=0}(p_i)$ have opposite monotonicity, we know there does not exist an interval for risklessly predictions. 

The above non-arbitrage opportunity is \emph{ex-post}, but the arbitrage opportunity persists when agents evaluate the conditional expectation of his score with respect to the random flipping step (which is the same as \textsf{WSWM}), which remains a concern when each agent participates in multiple event forecasts. This concern will be resolved when we apply the idea of surrogate wagering to the non-arbitrage wagering mechanism (\textsf{NAWM}). For details please refer to Section~\ref{sec:snawm}~~.

For \textsf{RP-SWME}, it runs \textsf{SWME} on each pair of agents after the random partition. Therefore, agents also have no arbitrage opportunity. 
~\\

\underline{(h) Pareto-optimality (\textsf{RP-SWME})}

In \textsf{RP-SWME}, any pair of agents with different beliefs has a positive probability to be partitioned into a sub-group.  Applying Lemma~2, at least one of them loses all his wager in the worst case. Thus,  by Definition~7, \textsf{RP-SWME} is PO.

%We prove that under \textsf{RP-SWME}, $\forall \report{},\mathbf{w}$, $\underline{\Pi}_i(\report{}, \mathbf{w}) < w_i$ for at most one agent $i$.  
%We first prove it by contradiction when $N\ne 3$. Suppose there are two agents $i$ and $j$ such that $\pi^{w}_i(\report{}, \mathbf{w})<w_i $ and $\pi^{w}_j(\report{}, \mathbf{w}) < w_j$. When $N\ne 3$, according to our random partition algorithm, there is a positive probability that agent $i$ and agent $j$ are paired together to participate in a \textsf{SWME} with an error rate that makes at least one of them lose all the wagers in the worst case, which contradicts with  $\pi^{w}_i(\report{}, \mathbf{w})<w_i\wedge\pi^{w}_j(\report{}, \mathbf{w})< w_j$. 

%When $N=3$, we can slightly change the random partition algorithm of the \textsf{RP-SWME} that we just randomly select two agents to participate in a surrogate \textsf{WSWM} with the adjust error rate. By such a way, each agent has a positive probability to be paired with another. Thus, our argument above still holds. 
%\end{proof}
\end{proof}
\subsection{Derivation of $\mathbb P(\tilde{X}_i = 1| X=0)$ and $\mathbb P(\tilde{X}_i = 0| X=1)$}

\begin{proof}
\begin{align*}
&\mathbb P(\tilde{X}_i = 1| X=0) = \mathbb P(\tilde{X}_i = 1, \hat{X} = 0| X=0)+\mathbb P(\tilde{X}_i = 1, \hat{X} = 1| X=0)\\
=&\mathbb P(\tilde{X}_i = 1| \hat{X} = 0, X=0) \cdot \mathbb P(\hat{X}=0|X=0) +\mathbb P(\tilde{X}_i = 1| \hat{X} = 1, X=0) \cdot \mathbb P(\hat{X}=1|X=0) \\
=&e^i_0 \cdot (1-\hat{e}_0)+(1-e^i_1) \cdot \hat{e}_0
%&=e_0 + (1-e_1-e_0) \cdot \hat{e}_0
\end{align*}
The third equality is due to conditional independence between $\tilde{\mathbf{X}}$ and $X$, given $\hat{X}$. Similarly we have 
$
\mathbb P(\tilde{X}_i = 0| X=1) =e^i_1 \cdot (1-\hat{e}_1)+(1-e^i_0) \cdot \hat{e}_1.
$
\end{proof}

